Efficient Parallel Output-Sensitive Edit Distance

Given two strings $A[1..n]$ and $B[1..m]$, and a set of operations allowed to edit the strings, the edit distance between $A$ and $B$ is the minimum number of operations required to transform $A$ into $B$. Sequentially, a standard Dynamic Programming (DP) algorithm solves edit distance with $\Theta(nm)$ cost. In many real-world applications, the strings to be compared are similar and have small edit distances. To achieve highly practical implementations, we focus on output-sensitive parallel edit-distance algorithms, i.e., to achieve asymptotically better cost bounds than the standard $\Theta(nm)$ algorithm when the edit distance is small. We study four algorithms in the paper, including three algorithms based on Breadth-First Search (BFS) and one algorithm based on Divide-and-Conquer (DaC). Our BFS-based solution is based on the Landau-Vishkin algorithm. We implement three different data structures for the longest common prefix (LCP) queries needed in the algorithm: the classic solution using parallel suffix array, and two hash-based solutions proposed in this paper. Our DaC-based solution is inspired by the output-insensitive solution proposed by Apostolico et al., and we propose a non-trivial adaption to make it output-sensitive. All our algorithms have good theoretical guarantees, and they achieve different tradeoffs between work (total number of operations), span (longest dependence chain in the computation), and space. We test and compare our algorithms on both synthetic data and real-world data. Our BFS-based algorithms outperform the existing parallel edit-distance implementation in ParlayLib in all test cases. By comparing our algorithms, we also provide a better understanding of the choice of algorithms for different input patterns. We believe that our paper is the first systematic study in the theory and practice of parallel edit distance.

==> code_bfssa.tex <==
\begin{algorithm}[htb]
\fontsize{9pt}{9pt}\selectfont
\caption{\small The BFS-based parallel edit distance algorithm\label{algo:lis-weighted}}

\KwIn{Two sequences $A_{1..n}$ and $B_{1..m}$.}
\KwOut{The edit distance between $A$ and $B$}
    \vspace{0.5em}

% To define a function, use:
% \SetKwProg{MyFunc}{Function}{}{end}
% To define a keyword, use:
% \newcommand{\Int}{\KwSty{int}}
% To define a for-loop, use:
% \SetKwFor{parForEach}{parallel\_for\_each}{do}{endfor}

\DontPrintSemicolon
$p\gets$\longestprefix$(A_{1..n},B_{1..m})$\\
$\ff_0=\{\langle p,p\rangle\}$\tcp*[f]{start from the longest }\\
$r\gets 0$ \tcp*[f]{$r$ is the current round (edit distance)}

\While {$\neg\,\visited[n,m]$} {
  %\lparForEach{$i\gets -r$ to $r$ } {$\diag[i]\gets 0$}
  $\diag[i]\gets 0$ for all $-r\le i\le r$ \tcp*[f]{$\diag[i]$: the last point on diagonal $i$}\\
  \parForEach{$\langle x,y \rangle \in \ff_i$}{
    \ForEach {$\langle \dx, \dy \rangle \in \{\langle0,1\rangle,\langle1,0\rangle \langle1,1\rangle\}$} {
      %$x'\gets x+\dx$\\
      %$y'\gets y+\dy$\\
      $\langle x', y'\rangle \gets \langle x+\dx, y+\dy \rangle$\\
      $p\gets$\longestprefix$(A_{x'..n},B_{y'..m})$\\
      \If {$\neg \,\visited[x'+p,y'+p]$} {
        %\tcp*[f]{Insert the new point $\langle x'+p, y'+p\rangle$ into the hash table using the key as $x'-y'$}
        %$\hashtable$.\textsc{Insert}$(x'-y', \langle x'+p, y'+p\rangle)$
        \tcp{for each diagonal, only keep the last element}
        $\diag[x'-y']\gets$ \writemax$(\diag[x'-y'], x)$
      }
      %$\ff_{r+1}\gets \{ \langle \diag[i],\diag[i]-i \rangle : -r\le i\le r \}$\\
      \parForEach{$-r\le i\le r$}{
        $\visited[i]\gets $\true\\
        \tcp{Put each point in $\diag[i]$ to the next frontier}
        $\ff_{r+1}[r+i] \gets \langle \diag[i],\diag[i]-i \rangle$
      }
      $r\gets r+1$
    }
  }
  \Return{$r$}
}
\yihan{There seems to be some issue in the code.}
\end{algorithm} 

==> code_bfssa2.tex <==
\begin{algorithm}[htb]
  \fontsize{9pt}{9pt}\selectfont
  \caption{\small The BFS-based parallel edit distance algorithm on two strings $A[1..n]$ and $B[1..m]$ \label{algo:bfs_in_code}}

  %\KwIn{Two sequences $A_{1..n}$ and $B_{1..m}$.}
  %\KwOut{The edit distance between $A$ and $B$}
      %\vspace{1pt}

  \DontPrintSemicolon
%diagonal id, for coordinate $(x,y)$, the diagonal id is $x-y$
  $f[i]\gets 0$ for all $-m\le i\le n$\tcp*[f]{$f[i]$ is the row-id of the last cell explored on diagonal $i$}\\
  $f[0]\gets$\longestprefix$(A[1..n],B[1..m])$\\
  $k\gets0$\tcp*[f]{$k$ is the edit distance}\\
  \While {$f[n-m]<n$\yihan{I didn't understand this condition}} {
    $k\gets k+1$\\
    \parForEach(\tcp*[f]{For diagonal $i$, find the cell in the new frontier}){$-k\le i \le k$}{ 
      \ForEach(\tcp*[f]{Enumerate three directions where the DP value comes from}) {$\langle\dx,\dy\rangle\in\{\langle0,1\rangle,\langle1,0\rangle,\langle1,1\rangle\}$} {
        $j\gets i-dx+dy$\tcp*[f]{when it is from direction $(dx,dy)$, the previous cell must from diagonal $j$ }\\
        %\tcp*[f]{assume the new cell on diagonal $i$ is $(x,y)$, since $i=x-y$, then $j=(x-dx)-(y-dy)=i-dx+dy$}
        \If {$-k+1\le j\le k-1$} {
          The row id $x\gets f[j]+dx$\\
          The column id $y\gets x-i$\\
          $p\gets$\longestprefix$(A[x+1..n],B[y+1..m])$\tcp*[f]{skip the common prefix}\\
          $g[i]=\max(g[i],x+p)$ \tcp*[f]{Keep the largest row id}\\
        }
      }
    }
    \parForEach{$-k\le i \le k$}{
      $f[i]=g[i]$
    }
  }
  \Return{$k$}\\
\end{algorithm} 

==> figures/bfs_exp.tex <==
\begin{figure*}[t]
    \centering
    \vspace{-1.0em}
    \includegraphics[width=\columnwidth]{figures/bfs_draft.pdf}
    \vspace{-1.2em}
    \caption{\textbf{The illustrations of the BFS process} \label{fig:bfs}}
    \vspace{-1.5em}
  \end{figure*}

==> figures/dp_table.tex <==
% \begin{figure*}[htb]
%     \centering
%     \includegraphics[width=0.5\columnwidth]{figures/bfs-figure.pdf}
%     \caption{\textbf{Traversing dynamic table} \label{fig:dp_table}}
%   \end{figure*}

  
  % \begin{figure}

  %   \begin{minipage}{0.45\textwidth}
  %   \begin{algorithm}[H]
  %   \hsize=\textwidth % <--------- THE HACK!
  %   \caption{Auto-entrenamiento}
  %   \label{alg_self}
  %   \begin{algorithmic}
  %   \State $m_0 \gets \textit{entrenar\_modelo}(\mathcal{D}_{l})$
  %   \Repeat
  %       \State $m \gets \textit{entrenar\_modelo}(\mathcal{D}_{l})$
  %       \For {$x \in \mathcal{D}_{u}$}
  %           \If {max $m(x) > \tau$}
  %               \State $\mathcal{D}_{l} \gets \mathcal{D}_{l} \cup \{(x, p(x))\}$
  %           \EndIf
  %       \EndFor
  %   \Until {las predicciones no sean confiables}
  %   \end{algorithmic}
  %   \end{algorithm}
  %   \end{minipage}\hfill
  %   \begin{minipage}{0.45\textwidth}
  %       \centering
  %       \includegraphics[width=0.5\columnwidth]{figures/bfs-figure.pdf}
  %       \caption{\textbf{Traversing dynamic table} \label{fig:dp_table}}
  %       \vspace{0.1cm} 
  %       \label{fig:ssl_self}
  %   \end{minipage}
  %   \end{figure}
    

==> imp-hash.tex <==
\subsection{Implementation details of Hashing Sparse Table}
\yihan{Maybe we can just remove this section? It doesn't contain much new compared to algorithm description.}
\youzhe{makes sense. Removed}
% Here we give some details of the parallel implementation of \hashtab{} building for
% LCP query.

% The hashing function we use to encode a truncated subsequence block $A[i + 1..i + b]$ is computed as
% $int(A[i + 1]) \times p^{b - 1} + int(A[i + b])$, where $p$ is a prime number corresponding to the character encoding space $\alpha$.
% For ASCII Codes including extended marks, the value of $\alpha$ is 256. Noticed that for any $p$, when the block
%  size is large, the total hashing value of this block maybe larger than integer space. Instead of applying module
%   operation on the present sum, we let the integer overflow natually, which avoids additional calculation.

% Instead of a rolling hashing way in Rabin-Karp to the calculation of \hashtab{}, a faster approach is to compute
% and store the  hash value of the blocks in parallel. The remaining layers of the table  with size $b \times 2^{1}, \cdots, b \times 2^{\log n}$
% of the table can be finished in parallel in order. The needed values for the computation can be
% directly looked up in the previous table layer, multiplied by predetermined power value.

% The auxiliary array $\suffixhash{A}$ for pre-computed suffix hashing value can also be finished in parallel, which supports
% the following comparison algorithm. 

